From Complex to Simple: Enhancing Multi-Constraint Complex Instruction Following Ability of Large Language Models

It is imperative for Large language models (LLMs) to follow instructions with elaborate requirements (i.e. Complex Instructions Following). Yet, it remains under-explored how to enhance the ability of LLMs to follow complex instructions with multiple constraints. To bridge the gap, we initially study what training data is effective in enhancing complex constraints following abilities. We found that training LLMs with instructions containing multiple constraints enhances their understanding of complex instructions, especially those with lower complexity levels. The improvement can even generalize to compositions of out-of-domain constraints. Additionally, we further propose methods addressing how to obtain and utilize the effective training data. Finally, we conduct extensive experiments to prove the effectiveness of our methods in terms of overall performance and training efficiency. We also demonstrate that our methods improve models' ability to follow instructions generally and generalize effectively across out-of-domain, in-domain, and adversarial settings, while maintaining general capabilities.

==> 010intro_bkp.tex <==
\input{figures/010intro}
% Instruction following很重要
Large language models (LLMs) have become the backbone for real-world applications~\cite{anil2023palm, touvron2023llama, achiam2023gpt}.
One of the key reasons is that LLMs can solve unseen tasks based on natural language instructions with few or no examples~\cite{brown2020language}.
The capability of LLMs to accurately understand instructions and convey the desired output, known as \textit{Instruction Following}~\cite{lou2024comprehensive}, is crucial for the safety~\cite{mu2023can} and reliability~\cite{zhou2023instruction} of LLMs.

\input{figures/010method}

% [jiaqing] 这两个视角可以吗
It is imperative for LLMs to follow instructions with elaborate requirements~\cite{yin2023llm, xu2023wizardlm} (i.e. \textit{Complex Instructions}), such as formatting and semantic specifications outlined in Fig. \ref{fig:010intro}.


First, end-users prefer detailed task descriptions over annotating samples~\cite{lou2024comprehensive, zhang2023tell}.
Additionally, certain tasks can be highly intricate and therefore costly and challenging to annotate, such as those in agent scenarios~\cite{zeng2023agenttuning}.
This underscores the importance of enabling LLMs to understand intricate task descriptions.
From a research perspective, the inherent research question behind complex instruction following is task generalization~\cite{yin2023llm}: whether LLMs can solve unseen tasks in low/zero-shot scenarios, considering that complex instructions hardly appear in the training dataset~\cite{zhou2024lima}. 

Specifically, complex instructions can be defined as instructions composing verifiable constraints~\cite{jiang2023followbench, qin2024infobench, he2024can}, such as semantic, numerical, and format constraints, as shown in Fig.~\ref{fig:010intro}.
Whether models can satisfy the constraints in the instructions (i.e. \textit{Constraints Following}) showcases their ability to follow instructions for two reasons:
(1) Human instructions are subjective and ambiguous while incorporating constraints ensures automatic evaluation of instruction following ability~\cite{zhou2023instruction, wang2024instructions}. 
(2) The compositional nature of constraints enables the creation of evaluation data without data leakage, thus effectively assessing the model's ability to generalize to unseen tasks~\cite{aksu2023cesar, zhou2023controlled}.

Complex constraints following is a challenging task for LLMs~\cite{jiang2023followbench, he2024can, qin2024infobench}.
As shown in Fig.~\ref{fig:010intro}, even advanced LLMs struggle to meet the four specified constraints in complex instructions.
However, it remains under-explored \textit{how to enhance LLMs to follow multi-constraint complex instructions}.
First, the existing works on constraints following mainly focus on \textit{evaluation} without proposing methods for enhancement~\cite{jiang2023followbench, chen2024benchmarking, xia2024fofo}.
Additionally, even when the improvement methods are proposed, they mainly consider instructions with \textit{few} constraints, thereby failing to showcase the complexity of human instructions in practical applications~\cite{chen2022controllable, zhang2023tell,  wang2024instructions}.
Moreover, although some studies construct complex instructions with multiple constraints and fine-tune LLMs on them~\cite{aksu2023cesar, sun2024conifer}, 
one key research question remains under-explored: \textbf{What \textit{training data} is effective in enhancing complex constraint-following abilities? }
This leads to two follow-up questions:
(1) \textbf{How to \textit{obtain} the effective training data?} and
(2) \textbf{How to \textit{utilize} the data effectively?}

% they only utilize positive samples via supervised fine-tuning (SFT).
% However, minor variations in complex instructions (e.g. adjusting numerical constraints from two to three in Fig.~\ref{fig:010intro}) can yield significant changes in output.
% We argue that using only positive samples via SFT inadequately and inefficently captures this distinction.

% First, the existing instruction tuning datasets mainly consist of common instructions~\cite{taori2023stanford, chiang2023vicuna}.
% Consequently, models trained on such data can hardly generalize to more complex instructions~\cite{jiang2023followbench}.
% Additionally, some studies gather complex instructions and train models using supervised fine-tuning (SFT)~\cite{aksu2023cesar, sun2024conifer}.
% However, minor variations in complex instructions (e.g. adjusting numerical constraints from two to three in Fig.~\ref{fig:010intro}) can yield significant changes in output.
% We argue that using only positive samples via SFT inadequately and inefficently captures this distinction.





% However, following instructions with multiple constraints is a challenging task for LLMs~cite{}. The reasons are as follows. First, the existing instruction tuning dataset mainly contains common instructions, ~\cite{}. Additionally, some researches collect complex instructions via humans or advanced LLMs, and tune models via next-word-prediction paradigm. Howver, as shown in \zj{xxx}, the slight changes in the complex instructions may lead to significant difference in the output. We argue that the next-word-prediction genertaion paradigm is hard to model this distinction.

% [jiaqing] 感觉写得有点weak

In this work, we systematically study how to enhance the ability of LLMs to follow complex instructions, with the framework shown in Fig.~\ref{fig:010method}.
We initially explore the effective training data for this purpose through an empirical study. 
We found that training LLMs on instructions containing multiple constraints (\textit{compositional data}) enhances their understanding of complex instructions more effectively than training on atomic constraints (\textit{atomic data}).
Moreover, the improvement in performance is related to the number of constraints, the model size (\S\ref{sec:emp}), and can even generalize to the compositions of out-of-domain constraints found in \S\ref{sec:050ood}.

To obtain high-quality compositional data, we generate initial output via a student model (vanilla model) and then correct via a teacher model (advanced model), termed the Discrimination method.  
This approach yields higher-quality output than using the teacher model to generate directly.
To leverage the positive and negative samples collected during the Discrimination method, we introduce a contrastive method with reinforcement learning fine-tuning (RLFT)~\cite{rafailov2023direct}. 
Our method surpasses the SFT training paradigm on the instruction following benchmark~\cite{zhou2023instruction} with fewer training steps. 
It also demonstrates superior generalization across out-of-domain, in-domain, and adversarial settings while preserving overall capabilities.


% We found that the generated output has better quality than the output generated via teacher model directly, defined as generation method.
% To better utilize the positive and negative samples collected via our discrimination method, we propose a contrastive method using reinforcement learning fine-tuning (RLFT). 
% Our method outperforms SFT training paradigm on the instruction following benchmark~\cite{zhou2023instruction} and requires fewer training steps.
% Moreover, our method has better generalization abilities under out-of-domain, in-domain, adversarial settings and also preserves general abilities.


% these research questions and found that:
% (1) Training LLMs on instructions containing multiple constraints (compositional data) enhances their understanding of atomic constraints or varying composition of constraints more effectively compared to training on atomic constraints (atomic data).
% Additionally, the generalization ability is related to the number of constraints and the model size.
% (2) For complex instructions, refining the output generated by a vanilla model with a more advanced model (discrimination method) enhances the ability to follow complex instructions more effectively than generating output directly from the advanced model (generation method).


% A common approach to enhance complex instruction following ability is to construct corresponding instances and fine-tune LLMs on them~\cite{aksu2023cesar, sun2024conifer}.
% Yet, one key research question remains under-explored: \textbf{What training data effectively enhances complex constraint-following abilities? }
% This leads to two follow-up questions:
% (1) How to \textbf{obtain} the effective training data, and
% (2) How to \textbf{utilize} it effectively?


% two key research questions remain under-explored:
% (1) What training data is effective?
% (2) How to obtain high-quality training data?

% We believe this is because slight changes in the instruction (i.e. constraint) can cause substantial output differences, which the discrimination-based method captures better than the next-word-prediction generation paradigm.

% Based on these findings, we propose a contrastive method using reinforcement learning fine-tuning (RLFT). 
% Specifically, we utilize an improved Direct Preference Optimization (DPO)~\cite{rafailov2023direct} to leverage both positive and negative samples collected during the discrimination method.
% By effectively using positive and negative contrastive pairs, our method outperforms SFT training paradigm on the instruction following benchmark~\cite{zhou2023instruction} and requires fewer training steps.
% Moreover, our method has better generalization abilities under out-of-domain, in-domain, adversarial settings and also preserves general abilities.

Overall, our contributions are mainly three-fold:
(1) We systematically improve LLMs' instruction-following ability by exploring effective training data.
(2) We design a discrimination-based method to obtain effective training data. We also propose a method for utilizing positive and negative samples obtained through this approach.
(3) We conduct extensive experiments to prove the effectiveness and efficiency of our method. We also validate its generalization ability under four settings.


% (1) we systematically study how to improve LLMs' ability to follow instructions, including training data 应该include atomic constraints 还是compositional constraints, training paradigm应该是generation还是discrimination. (2) We propose a constraive learning framework, which outperforms the next-word-prediction generation paradigm and requires fewer training steps. (3) We conduct extensive experiments to prove the effectiveness of our method, including the generazalition abilities on more challenging complex instruction and unseen phrasing, while preserving the models' general ability.

% In this work, we systematically study how to enhance complex instructions following ability of LLMs. Initially, we conduct two emprical studies. We found that (1) Training on instructions containing multiple constrains (compositional data) can enhance models understand atomic constraints or varying compositional data spontaneously compared to training on atomic constraints individually. (2) For the complex instruction, the output generated by the vanilla model subsequently refined by more advanced model (discrimination method), follows complex instructions more effectively than the output generated directly by the teacher model (generation method). Consequently, we propose a contrastive learning framework, which adopts improved DPO to leverage both positive and negative samples collected during discrimination method. Finally, our framework performs better than the next-word-prediction paradigm on the instruction following benchmark. Also, our framework has better generalization ability on more challenging complex instructions, unseen phrasing while retain the model's general ability.
% [to do]收敛更快
% 因此，我们系统地研究了如何增强模型的复杂指令理解能力。我们首先进行了两个emprical studies，发现（1）（2）。接着，我们提出了contrastive-based的训练方式，让模型更好地捕捉微小的改变对结果的影响

==> 020related_bkp.tex <==
\subsection{Evaluation of Instruction Following}
% Large language models (LLMs) have become the backbone for real-world applications, one of the key reasons is that LLMs can solve tasks with natural language instructions. The capability of LLMs to accurately understand instructions and convey the desired output, known as instruction following, is crucial for the 实用性、safety and reliability of LLMs.
% Large language models (LLMs) have become the backbone of real-world applications, largely due to their ability to understand natural language instructions, ranging from casual conversation to complex problem solving~\cite{}.
Unlike traditional example-driven supervision, Large Language Models (LLMs) can understand task descriptions (i.e. instructions) with few or no examples~\cite{}.
The ability to accurately understand instructions and convey the desired output is imperative for ensuring the practicality and safety of LLMs, termed as \textit{Instruction Following}~\cite{}.
% The fundamental research question behind Instruction Following is Generalization: can model generalize to unseen task in few-shot/zero-shot setting. A line of work 通过对答案空间进行扰动，评估模型是truly understand instructions or simply recite the answer. Another line of work通过constraints following为代表测试模型的Instruction following的能力的，as constraints是客观的、可验证的。
There are various perspectives for assessing the ability of LLMs to follow instructions.
A line of work perturbs the answer space to assess whether the model truly understands instructions or recites the answer~\cite{}. 
Another line of work exemplifies models' ability to follow instructions by incorporating verifiable constraints within them~\cite{}.
% such as lexical~\cite{}, length~\cite{}, format~\cite{}, and semantic~\cite{} constraints.
% The compositional nature of these constraints allows one instruction to include multiple constraints simultaneously.
% 这种同时包含多种constraints的复杂指令在practical use中经常出现，为LLMs提出了更大的挑战。
% These \textit{complex instructions} containing multiple user-specified constraints often arise in practical use, posing greater challenges for LLMs~\cite{}.
% Our work belongs to the latter one. 然而constraints following的工作普遍存在两个问题（1）只有evaluation，没有提出优化的方法（2）即使提出优化的方法，仅考虑了单条约束，不能反映真实使用过程中指令的复杂性。Different from these work, our work以多条约束组合的复杂指令为例，提出了优化LLM遵循复杂指令的框架。
Our work belongs to the latter category. 


% the ability to accurately understand task semantics and convey the desired output makes them perform well on the few-shot/zero-shot tasks, which 
% The ability of LLMs to accurately understand instructions and convey the desired output, termed \textit{Instruction Following}, is imperative for ensuring the practicality and safety of LLMs~\cite{}.

% Existing studies从不同角度衡量模型遵循指令的能力，包含模型



\subsection{Constrained Text Generation for LLMs}
% Complex Instruction Following的定义：和传统的Controlled Text Generation不同，Instruction是人类的表述，更加多样
% 主要研究为Evaluation
% 一些工作关注Enhancement
% 从数据层面，只考虑了单种、单条的约束，但实际场景是多种、多条约束集合的复杂指令。
% 从方法层面，没有系统性地研究什么样的训练数据和范式对Instruction following的能力有帮助。
% In this work, 大模型control their generation去satisfy user-specified constraints被定义为Complex Instruction Following的能力。
% 感觉需要提下游任务
% verifiable只是一个桥梁

% Many studies发现大模型很难meet user-specified constraints, such as lexical, length, and format constraints.
% Due to the composition of these constraints，指令可以同时包含多种constraints，模型表现会进一步下降。
% Recently，许多工作希望提升模型同时遵循多种constraints的表现效果，as defined as Complex Instruction Following in this work.
% Many works construct instances that satisfy constraints and fine-tuning language models on these instances. Other works modify the attention scores to 让模型关注到特定的约束。
Many studies have found that large language models struggle to meet specified constraints in instructions, such as lexical~\cite{}, length~\cite{}, format~\cite{}, and semantic~\cite{} constraints.
The compositional nature of these constraints allows one instruction to include multiple constraints simultaneously~\cite{}.
% % 这种同时包含多种constraints的复杂指令在practical use中经常出现，为LLMs提出了更大的挑战。
These \textit{complex instructions} containing multiple user-specified constraints often arise in practical use, posing greater challenges for LLMs~\cite{}.

These works have three main limitations.
Firstly, they solely focus on evaluation without proposing methods for enhancement~\cite{}.
Also, even when the improvement methods are proposed, they only consider instructions with a few constraints, thereby failing to showcase the complexity of human instructions in practical applications~\cite{}.
Moreover, many studies create instances that satisfy multiple constraints and fine-tune language models accordingly~\cite{}.
We argue that the next-word-prediction paradigm fails to guide models effectively toward the specified constraints, especially when instructions incorporate multiple constraints.
Different from existing works, we introduce a framework that utilizes instructions with multiple constraints as examples, aiming to enhance the capability of LLMs to understand and follow complex instructions effectively.
% Many studies create instances satisfying specific constraints and fine-tune language models on them~\cite{}. 
% Others adjust attention scores to direct the model's focus toward the specified constraints~\cite{}.





\subsection{Tuning with Complex Instructions}
Complex Instructions refer to instructions that involve more reasoning steps~\cite{}, intricate input~\cite{}, or additional constraints~\cite{}.
Many studies have demonstrated that fine-tuning with complex instructions can enhance a model's performance on instruction following~\cite{}, reasoning~\cite{}, and code generation~\cite{}.
The complex instructions are either written by humans~\cite{} or rewritten by teacher model~\cite{}.
Our works have two main differences from these works.
First, we focus on improving LLMs' ability to follow complex instructions, ...
Instead of directly fine-tuning on these  we propose a framework ....

% The high-quality data either 来自于人类筛选、

% 普遍的观点是，越高质量的数据会有更佳的效果
% 人工筛选（Lima、FollowBench）、ChatGPT改写（orca、wizardLM、wizardMath）

















==> figures/010emprical_followbench.tex <==
\begin{figure*}[t] 
    \centering
        \includegraphics[width=0.8\textwidth]{figures/files/followbench.pdf}
    % \captionsetup{font={small}} 
    \caption{TODO}
    \label{fig:010followbench}
\end{figure*}


==> figures/050ood.tex <==
\begin{figure}[t] 
    \centering
        \includegraphics[width=1\linewidth]{figures/files/ood.pdf}
    % \captionsetup{font={small}} 
    \caption{\hqy{The performance on Followbench (left) and CELLO (right). D and C denote Ours-13B-Discrimination and Ours-13B-Contrastive respectively.
    }}
    \label{fig:050ood}
\end{figure}


==> tables/050followbench.tex <==
\newcolumntype{b}{>{\columncolor{blue!10}}r}
% \newcolumntype{d}{>{\columncolor{brown!10}}r}
% \newcolumntype{q}{>{\columncolor{Green!10}}r}


\setlength\tabcolsep{9pt}
\begin{table*}[!htb]
  \centering
  \tiny
    \resizebox{0.95\textwidth}{!}{
\begin{tabular}{lcccccb}

\toprule

\textbf{Models}  & \textbf{Level 1} & \textbf{Level 2} & \textbf{Level 3} & \textbf{Level 4} & \textbf{Level 5} & \textbf{Total} \\

\midrule                    
    

LlaMA2-13B-chat          & 49.86   & 48.35   & 41.70   & 35.49   & 34.78   & 42.04 \\
$Ours$-13B-$generation$  & 56.29   & 53.12   & 41.44   & 33.20   & 28.09   & 42.43 \\
$Ours$-13B-$contrastive$ & 53.22   & 52.21   & 47.25   & 33.35   & 27.81   & 42.77 \\

\bottomrule
\end{tabular}
}
  \caption{
  (TODO) The HSR of models on FollowBench. Level $x$ indicates there are $x$ constraints in the instructions.
  }
  \label{tab:050followbench}
\end{table*}

==> tables/050generalization_desp.tex <==
% \newcolumntype{b}{>{\columncolor{blue!10}}r}
\newcolumntype{d}{>{\columncolor{brown!10}}r}
\newcolumntype{q}{>{\columncolor{Green!10}}r}


\setlength\tabcolsep{1pt}
\begin{table*}[!htb]
  \centering
  \large
    \resizebox{0.95\textwidth}{!}{
\begin{tabular}{lcccccccccdb}

\toprule

\textbf{Models} & \textbf{ChangeCase} & \textbf{Combination} & \textbf{Content} & \textbf{Format} & \textbf{Keywords} & \textbf{Language} & \textbf{Length} & \textbf{Punctuation} & \textbf{Startend} & \textbf{I-level} & \textbf{C-level} \\

\midrule                    
    
LLaMA2-13B-Chat                 &17.86 & 00.00  & 68.42 & 58.54 & 61.43 & 27.27  & 34.43 & 00.00  & 27.03 & 09.50  & 42.27 \\
WizardLM-13B-V1.2               &16.67 & 13.64  & 56.58 & 53.66 & 64.29 & 100.00 & 40.98 & 17.39 & 48.65 & 14.00 & 47.20 \\
OpenChat-13B-V3.2               &25.00 & 00.00  & 76.32 & 56.71 & 61.43 & 86.36  & 35.25 & 15.22 & 55.41 & \underline{16.50} & 49.07 \\
\cdashlinelr{1-12}
$\text{Ours-LLaMA2-13B}_\text{Discrimination}$    &48.81 & 00.00  & 67.11 & 50.61 & 58.57 & 90.91  & 36.89 & 60.87 & 67.57 & 15.00 & \underline{53.33} \\
$\text{Ours-LLaMA2-13B}_\text{Contrastive}$   &35.71 & 04.55  & 63.16 & 50.61 & 65.00 & 86.36  & 47.54 & 63.04 & 79.73 & \textbf{19.00} & \textbf{55.73} \\

\bottomrule
\end{tabular}
}
  \caption{The performance of models on instructions within the same constraint category (each with 3 to 5 constraints) but with varying phrasing and detailed requirements, assessing our methods' in-domain generalization ability.
  }
  \label{tab:050desp}
\end{table*}

==> tables/050generalization_more.tex <==
% \newcolumntype{b}{>{\columncolor{Blue!10}}r}
\newcolumntype{d}{>{\columncolor{brown!10}}r}
\newcolumntype{q}{>{\columncolor{Green!10}}r}


\setlength\tabcolsep{1pt}
\begin{table*}[!htb]
  \centering
  \large
    \resizebox{0.95\textwidth}{!}{
\begin{tabular}{lcccccccccdb}

\toprule

\textbf{Models} & \textbf{ChangeCase} & \textbf{Combination} & \textbf{Content} & \textbf{Format} & \textbf{Keywords} & \textbf{Language} & \textbf{Length} & \textbf{Punctuation} & \textbf{Startend} & \textbf{I-level} & \textbf{C-level} \\

\midrule                    
    
LLaMA2-13B-Chat                 &25.71 & 08.70 & 67.44 & 47.41 & 60.71 & 28.00 & 26.92 & 02.38  & 21.90 & 01.00 & 40.15 \\
WizardLM-13B-V1.2               &28.57 & 00.00 & 54.26 & 50.00 & 66.67 & 72.00 & 34.62 & 15.48 & 52.38 & 07.00 & 46.60 \\
OpenChat-13B-V3.2               &31.43 & 04.35 & 62.79 & 56.03 & 60.71 & 72.00 & 31.73 & 23.81 & 49.52 & \underline{07.30} & 47.64 \\
\cdashlinelr{1-12}
$\text{Ours-LLaMA2-13B}_\text{Discrimination}$     &51.43 & 04.35 & 57.36 & 35.34 & 65.48 & 48.00 & 31.25 & 59.52 & 69.52 & 05.00 & \underline{49.53} \\
$\text{Ours-LLaMA2-13B}_\text{Contrastive}$  &40.95 & 08.70 & 50.39 & 45.69 & 72.22 & 64.00 & 37.50 & 55.95 & 74.29 & \textbf{07.50} & \textbf{53.05} \\


\bottomrule
\end{tabular}
}
  \caption{The performance of models on more challenging complex instructions with 6 to 7 constraints. The adversarial setting stress tests the generalization ability of LLMs in following complex instructions.}
  \label{tab:050more}
\end{table*}

==> tables/100followbench_ckp0.tex <==
\newcolumntype{b}{>{\columncolor{blue!10}}r}
% \newcolumntype{d}{>{\columncolor{brown!10}}r}
% \newcolumntype{q}{>{\columncolor{Green!10}}r}


\setlength\tabcolsep{8pt}
\begin{table*}[!htb]
  \centering
  \tiny
    \resizebox{0.95\textwidth}{!}{
\begin{tabular}{lcccccb}

\toprule

category               & \textbf{Level 1} & \textbf{Level 2} & \textbf{Level 3} & \textbf{Level 4} & \textbf{Level 5} & \textbf{Total} \\
\midrule
content        & 44.00            & 44.00            & 40.00            & 40.00            & 40.00            & 41.60          \\
example        & 0.00             & 0.00             & 0.00             & 0.00             & 0.00             & 0.00           \\
format         & 70.00            & 70.00            & 63.33            & 46.67            & 40.00            & 58.00          \\
mixed          & 29.41            & 29.41            & 23.53            & 23.53            & 23.53            & 25.88          \\
situation      & 59.09            & 50.00            & 50.00            & 22.73            & 31.82            & 42.73          \\
style          & 96.67            & 96.67            & 73.33            & 80.00            & 73.33            & 84.00          \\
\midrule
\textbf{Total} & 49.86            & 48.35            & 41.70            & 35.49            & 34.78            & 42.04          \\

\bottomrule
\end{tabular}
}
  \caption{(TODO) HSR of LlaMA2-13B-chat across different constraints of different levels. Level $x$ indicates there are $x$ constraints in the instructions.
  }
  \label{tab:100followbench_ckp0}
\end{table*}

==> tables/100followbench_ckp2.tex <==
\newcolumntype{b}{>{\columncolor{blue!10}}r}
% \newcolumntype{d}{>{\columncolor{brown!10}}r}
% \newcolumntype{q}{>{\columncolor{Green!10}}r}


\setlength\tabcolsep{8pt}
\begin{table*}[!htb]
  \centering
  \tiny
    \resizebox{0.95\textwidth}{!}{
\begin{tabular}{lcccccb}

\toprule

category               & \textbf{Level 1} & \textbf{Level 2} & \textbf{Level 3} & \textbf{Level 4} & \textbf{Level 5} & \textbf{Total} \\
\midrule
content        & 56.00            & 52.00            & 40.00            & 32.00            & 24.00            & 40.80          \\
example        & 10.00            & 5.00             & 5.00             & 2.50             & 2.50             & 5.00           \\
format         & 83.33            & 73.33            & 63.33            & 36.67            & 36.67            & 58.67          \\
mixed          & 52.94            & 52.94            & 29.41            & 35.29            & 23.53            & 38.82          \\
situation      & 45.45            & 45.45            & 40.91            & 22.73            & 31.82            & 37.27          \\
style          & 90.00            & 90.00            & 70.00            & 70.00            & 50.00            & 74.00          \\
\midrule
\textbf{Total} & 56.29            & 53.12            & 41.44            & 33.20            & 28.09            & 42.43          \\

\bottomrule
\end{tabular}
}
  \caption{(TODO) HSR of $Ours$-13B-$discrimination$ across different constraints of different levels. Level $x$ indicates there are $x$ constraints in the instructions.
  }
  \label{tab:100followbench_ckp2}
\end{table*}

==> tables/100followbench_ckp3.tex <==
\newcolumntype{b}{>{\columncolor{blue!10}}r}
% \newcolumntype{d}{>{\columncolor{brown!10}}r}
% \newcolumntype{q}{>{\columncolor{Green!10}}r}


\setlength\tabcolsep{8pt}
\begin{table*}[!htb]
  \centering
  \tiny
    \resizebox{0.95\textwidth}{!}{
\begin{tabular}{lcccccb}

\toprule

category       & \textbf{Level 1} & \textbf{Level 2} & \textbf{Level 3} & \textbf{Level 4} & \textbf{Level 5} & \textbf{Total} \\
\midrule
content        & 56.00            & 52.00            & 44.00            & 40.00            & 24.00            & 43.20          \\
example        & 10.00            & 5.00             & 5.00             & 2.50             & 2.50             & 5.00           \\
format         & 76.67            & 63.33            & 60.00            & 46.67            & 40.00            & 57.33          \\
mixed          & 41.18            & 52.94            & 41.18            & 29.41            & 17.65            & 36.47          \\
situation      & 45.45            & 50.00            & 50.00            & 18.18            & 22.73            & 37.27          \\
style          & 90.00            & 90.00            & 83.33            & 63.33            & 60.00            & 77.33          \\
\midrule
\textbf{Total} & 53.22            & 52.21            & 47.25            & 33.35            & 27.81            & 42.77         \\

\bottomrule
\end{tabular}
}
  \caption{(TODO) HSR of $Ours$-13B-$contrastive$ across different constraints of different levels. Level $x$ indicates there are $x$ constraints in the instructions.
  }
  \label{tab:100followbench_ckp3}
\end{table*}

==> tables/100train_test_new.tex <==
% \newcolumntype{b}{>{\columncolor{Blue!10}}r}
\newcolumntype{d}{>{\columncolor{brown!10}}r}
\newcolumntype{q}{>{\columncolor{Green!10}}r}

\setlength\tabcolsep{4pt}
\begin{table*}[!htb]
  \centering
  \tiny
    \resizebox{0.5\textwidth}{!}{
\begin{tabular}{lccccccbcccccb}
\toprule
\multirow{2}{*}{Benchmark} & \textbf{} & \multicolumn{6}{c}{\textbf{Training Set}} & \multicolumn{6}{c}{\textbf{Test Set}} \\
\cmidrule(lr){3-8} \cmidrule(lr){9-14}
& & \textbf{L1} & \textbf{L2} & \textbf{L3} & \textbf{L4} & \textbf{L5} & \textbf{Avg.} & \textbf{L1} & \textbf{L2} & \textbf{L3} & \textbf{L4} & \textbf{L5} & \textbf{Avg.} \\
\midrule
\multirow{7}{*}{FollowBench} & Type & 31 & 20 & 17 & 16 & 16 & 100 & 9 & 20 & 23 & 24 & 24 & 100 \\
& content & 16 & 15 & 17 & 15 & 12 & 75 & 9 & 10 & 8 & 10 & 13 & 50 \\
& situation & 14 & 13 & 13 & 13 & 13 & 66 & 8 & 9 & 9 & 9 & 9 & 44 \\
& style & 19 & 19 & 18 & 18 & 16 & 90 & 11 & 11 & 12 & 12 & 14 & 60 \\
& format & 20 & 19 & 17 & 18 & 16 & 90 & 10 & 11 & 13 & 12 & 14 & 60 \\
& mixed & 14 & 10 & 11 & 7 & 6 & 48 & 3 & 7 & 6 & 10 & 11 & 37 \\
& Total & 114 & 96 & 93 & 87 & 79 & 469 & 50 & 68 & 71 & 77 & 85 & 351 \\
\midrule 
\multirow{2}{*}{IFEval} & One-cons & - & - & - & - & - & 92 & - & - & - & - & - & 213 \\
& Multi-cons & - & - & - & - & - & 92 & - & - & - & - & - & 144 \\
\bottomrule
\end{tabular}
}
  \caption{The statistic of the datasets used in the empirical study.}
  \label{tab:performance_comparison}
\end{table*}

